EPIC: Efficient Predicate-Guided Inference-Time Control for Compositional Text-to-Image Generation

Recent text-to-image (T2I) generators can synthesize realistic images, but still struggle with compositional prompts involving multiple objects, counts, attributes, and relations. We introduce EPIC (Efficient Predicate-Guided Inference-Time Control), a training-free inference-time refinement framework for compositional T2I generation. EPIC casts refinement as predicate-guided search: it parses the original prompt once into a visual program of object variables and typed predicates, then verifies each candidate image against this program using visual evidence extracted from that image. A candidate is judged to satisfy the prompt when all predicates pass; otherwise, unmet predicates guide the next step, routing localized failures to targeted editing and layout-level or persistent failures to resampling. On GenEval2, EPIC improves the prompt-level Soft-TIFA GM score from 34.16% for single-pass generation to 71.46%. With the same generator, editor, and image-model execution budget, EPIC outperforms the strongest baseline by 19.23 points. It also uses 31% fewer image-model executions, 72% fewer multimodal large language model (MLLM) calls, and 81% fewer MLLM tokens per prompt.

==> tables/geneval2/geneval2_atomicity.tex <==
\begin{table}[t]
\centering
\caption{GenEval2 prompt-level accuracy by atomicity at $T=0$.
\method{} improves prompt-level accuracy as compositionality increases,
especially from atomicity 5 to 10.
Best and second-best scores among FLUX.2-Klein-9B based methods are
shown in \textbf{bold} and \underline{underlined}, respectively.}
\label{tab:geneval2_atomicity}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabularx}{\linewidth}{lYYYYYYYY}
\toprule
Method & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\midrule

FLUX.2-Klein-9B
& 63.17 & 55.11 & 38.78 & 34.27
& 23.22 & 21.66 & 19.90 & 17.19 \\

\midrule
\multicolumn{9}{l}{\emph{Inference-time scaling with FLUX.2-Klein-9B}} \\

BoN+NVILA
& 75.72 & 64.70 & 52.05 & 44.12
& 28.06 & 28.03 & 23.64 & 16.49 \\

T2I-Copilot
& 64.33 & 59.15 & 45.68 & 44.42
& 25.35 & 19.37 & 19.53 & 14.64 \\

RAISE
& \second{82.52} & \second{74.92} & \second{59.92} & \second{55.62}
& \second{41.84} & \second{42.16} & \second{32.49} & \second{28.37} \\

\method{}
& \best{90.26} & \best{89.79} & \best{78.78} & \best{74.54}
& \best{68.45} & \best{62.78} & \best{57.70} & \best{48.02} \\
\bottomrule
\end{tabularx}
\end{table}

